Training Protocol Matters: Towards Accurate Scene Text Recognition via Training Protocol Searching

The development of scene text recognition (STR) in the era of deep learning has been mainly focused on novel architectures of STR models. However, training protocol (i.e., settings of the hyper-parameters involved in the training of STR models), which plays an equally important role in successfully training a good STR model, is under-explored for scene text recognition. In this work, we attempt to improve the accuracy of existing STR models by searching for optimal training protocol. Specifically, we develop a training protocol search algorithm, based on a newly designed search space and an efficient search algorithm using evolutionary optimization and proxy tasks. Experimental results show that our searched training protocol can improve the recognition accuracy of mainstream STR models by 2.7%~3.9%. In particular, with the searched training protocol, TRBA-Net achieves 2.1% higher accuracy than the state-of-the-art STR model (i.e., EFIFSTR), while the inference speed is 2.3x and 3.7x faster on CPU and GPU respectively. Extensive experiments are conducted to demonstrate the effectiveness of the proposed method and the generalization ability of the training protocol found by our search method. Code is available at https://github.com/VDIGPKU/STR_TPSearch.

==> tables/CvsT.tex <==
\begin{table}[]
\renewcommand\arraystretch{1.1}
\centering
\caption{Comparison of our CRNN~\cite{shi2017end} baseline and Transformer~\cite{vaswani2017attention} baseline when training with different searched training protocols. $T_{B}$, $T_{C}$ and $T_{T}$ represent baseline training protocol, training protocols searched by CRNN and Transformer, respectively. Optimal results for each model are shown in \textbf{bold} font.
\textit{Difference} means the difference accuracy between the two models. Different models do not have the same optimal training protocol. 
} % title of Table
\begin{tabular}{c|c|cc|c}
\hline
Model       & $T_{B}$ & $T_{C}$ & $T_{T}$ & $\Delta$Acc. \\ \hline
CRNN        & 84.3           & \textbf{88.2$^{+3.9}$}            & 87.3$^{+3.0}$ & -0.9             \\
Transformer & 81.7           & 85.3$^{+3.6}$            & \textbf{86.4$^{+4.7}$} & +1.1              \\ \hline
Difference  & 2.6            & 2.9                  & 0.9                  & -                \\
\hline
\end{tabular}
\label{table:CvsT}
\end{table}

==> tables/baseline.tex <==
% \begin{table}
% \centering
% %\small
% \caption{Comparison of different training methods. \textit{SP} denotes using our searched training protocol. \textit{TTS} represents using the proposed two-phase training scheme. } 
% \begin{tabular}{c|cc|cc}
% \hline
% \multirow{2}{*}{Model} & \multirow{2}{*}{SP}  & \multirow{2}{*}{TTS} & \multicolumn{2}{c}{Overall Accuracy(\%)}                          \\
%                       &                      &                      & Regular              & \multicolumn{1}{c}{Irregular} \\
% %\hline
% %\cite{baek2019wrong}&&&84.10\\
% \hline
% \multirow{2}{*}{Attention-based} 
% %${\surd}$ & ${\surd}$& ${\surd}$   &  & 86.73    \\
% &  & - &93.45 &78.31 \\%&88.11 \\
% & ${\surd}$  & - &\textbf{95.51(+2.06)} &\textbf{84.09(+5.78)} \\%&\textbf{91.49}$^{+3.38}$ \\
% \hline
% \multirow{3}{*}{CTC-based}      
% %${\surd}$ & ${\surd}$& ${\surd}$   &  & 86.73    \\
% &  &  &91.63 &75.58 \\%&85.97 \\
% & ${\surd}$  &   &94.34(+2.71) &81.46(+5.88) \\%&89.80$^{+3.83}$ \\
% & ${\surd}$  & ${\surd}$  &\textbf{95.32(+3.69)}  &\textbf{83.02(+7.44)} \\%&\textbf{90.98}$^{+5.01}$ \\
% \hline     
% \end{tabular}
% \label{table:baseline}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{c|cccc|c}
% \hline
%                      & MJ     & ST\_a   & ST     & Real   & Acc. \\ \hline
%                      & \cmark &        &        &        & 76.7 \\
%                      &        & \cmark &        &        & 65.4 \\
%                      &        &        & \cmark &        & 77.6 \\ \hline
% \cite{baek2019wrong} & \cmark & \cmark &        &        & 78.8 \\ 
%                      & \cmark &        & \cmark &        & 83.0 \\ \hline
% Baseline             & \cmark &        & \cmark & \cmark & 84.3 \\
% \hline
% \end{tabular}
% \label{table:baseline}
% \end{table}

\begin{table}[t]
\centering
\caption{Comparison between baseline and searched training protocols. Our search algorithm can be applied to both CRNN and Transformer baseline and the searched training protocols significantly improved their recognition accuracy.} 
\begin{tabular}{c|cc|c}
\hline
Model       & Baseline & Searched & $\Delta$Accuracy \\ \hline
CRNN        & 84.3     & 88.2     & +3.9              \\
Transformer & 81.7     & 86.4     & +4.7              \\\hline
\end{tabular}
\label{table:baseline}
\end{table}


